3D-Aware Video Generation

Generative models have emerged as an essential building block for many image synthesis and editing tasks. Recent advances in this field have also enabled high-quality 3D or video content to be generated that exhibits either multi-view or temporal consistency. With our work, we explore 4D generative adversarial networks (GANs) that learn unconditional generation of 3D-aware videos. By combining neural implicit representations with time-aware discriminator, we develop a GAN framework that synthesizes 3D video supervised only with monocular videos. We show that our method learns a rich embedding of decomposable 3D structures and motions that enables new visual effects of spatio-temporal renderings while producing imagery with quality comparable to that of existing 3D or video GANs.

==> public/tab/forensics_quantitative.tex <==
\begin{table}[ht!]
    \centering
    \begin{tabularx}{0.73\linewidth}{l|lccc}
        \toprule
        \multirow{2}{*}{Type} & \multirow{2}{*}{Method} & \multicolumn{3}{@{}c}{FaceForensics}\\
        %\cmidrule{1-4}
        & & FVD& FID & Training Time \\
        \midrule
        \multirow{1}{*}{2D Image} & StyleGAN2 \cite{Karras2020CVPR} & - & 8.4 & 7.5\\
        \midrule
        \midrule
        \multirow{5}{*}{2D Video}     & VideoGPT \cite{Yan2021ARXIV} & 185.9& 22.7 & 32 \\    & MoCoGAN \cite{Tulyakov2018CVPR} & 124.7& 24.0 & 5 \\
        & MoCoGAN-HD \cite{Tian2021ICLR} & 111.8 & 7.1 & 16.5\\
        
        & DIGAN \cite{Yu2022ICLR} & 62.5 & 19.1 & 16 \\
        & StyleGAN-V \cite{Skorokhodov2022CVPR} & 47.4 & 9.4 & 8 \\

        \midrule
        \multirow{1}{*}{3D Static}         & StyleNeRF \cite{Gu2022ICLR} & - & 16.2 & 7.5 \\
        \midrule
        \multirow{1}{*}{3D Video} & Ours & \todo{68.7} & \todo{13.7} & \todo{8} \\
        \bottomrule
    \end{tabularx}
    %\vspace{0.5em}
    \caption{{\bf{Quantitative Results on FaceForensics.}} We report FVD
    ($\downarrow$), FID ($\downarrow$) and the corresponding training time (in GPU days) for
    our baselines and our method at $256^2$ pixel resolution. All reported timings are measured on a machine with an NVIDIA V100.}
    \label{tab:vid_gen_sota_ff}
    %\vspace{-0.5cm}
\end{table}


%\begin{table}[!t]
%    \caption{SOTA comparison to 2D Video Generators on FaceForensics 256\textsuperscript{2} GPU-days}  
%    \label{tab:vid_gen_sota_ff}
%    \centering
%    \begin{tabularx}{0.75\linewidth}{@{}X@{}cccc@{}}
%        \toprule
%        \multirow{2}{*}{Method} & \multicolumn{3}{@{}c}{FaceForensics}\\
%        \cmidrule{2-4}
%         & FVD\textsubscript{16}& FID & Training Cost \\
%        \midrule
%        MoCoGAN \cite{Tulyakov2018CVPR} & 124.7& 24.0 & \textbf{5} \\
%        MoCoGAN w/ StyleGAN2 \cite{Skorokhodov2022CVPR} & 55.6 & 10.8 & 8 \\
%        MoCoGAN-HD \cite{Tian2021ICLR} & 111.8 & \textbf{7.1} & 16.5\\
%        VideoGPT \cite{Yan2021ARXIV} & 185.9& 22.7 & 32 \\
%        DIGAN \cite{Yu2022ICLR} & 62.5 & 19.1 & 16 \\
%        StyleGAN-V \cite{Skorokhodov2022CVPR} & \textbf{47.4} & 9.4 & 8 \\
%        \midrule
%        Ours & \todo{68.7} & \todo{13.7} & \todo{8} \\
%        \bottomrule
%    \end{tabularx}
%\end{table}
%
%\begin{table}[!t]
%    \caption{SOTA comparison to Image Generators on FaceForensics 256\textsuperscript{2} \todo{definately put in tab1}}
%    \label{tab:img_gen_sota}
%    \centering
%    \begin{tabularx}{0.25\linewidth}{@{}X@{}c@{}}
%        \toprule
%        Method & FID \\
%        \midrule
%        StyleGAN2 \cite{Karras2020CVPR} & 8.4 \\
%        StyleNeRF \cite{Gu2022ICLR} & \todo{x.x} \\
%        \midrule
%        Ours & \todo{x.x} \\
%        \bottomrule
%    \end{tabularx}
%\end{table}


==> public/tab/forensics_training_cost.tex <==
\begin{table}[!t]
    \centering
    \begin{tabularx}{0.55\linewidth}{l|lc}
        \toprule
        \multirow{1}{*}{Type} & \multirow{1}{*}{Method} & Training Time \\
        \midrule
        \multirow{1}{*}{2D Image} & StyleGAN2 \cite{Karras2020CVPR} & 7.5\\
        \midrule
        \multirow{5}{*}{2D Video}     & VideoGPT \cite{Yan2021ARXIV} & 32 \\    & MoCoGAN \cite{Tulyakov2018CVPR} & 5 \\
        & MoCoGAN-HD \cite{Tian2021ICLR} & 16.5\\
        
        & DIGAN \cite{Yu2022ICLR} & 16 \\
        & StyleGAN-V \cite{Skorokhodov2022CVPR} & 8 \\

        \midrule
        \multirow{1}{*}{3D Static}         & StyleNeRF \cite{Gu2022ICLR} & 7.5 \\
        \midrule
        \multirow{1}{*}{3D Video} & Ours & \todo{8} \\
        \bottomrule
    \end{tabularx}
    %\vspace{0.5em}
    \caption{{Training Costs on FaceForensics}. We report the corresponding training times (in GPU days) for
    our baselines and our method at $256^2$ pixel resolution. All reported timings are measured on a machine with NVIDIA V100 GPUs.}
    \label{tab:vid_gen_sota_ff_cost}
    %\vspace{-0.5cm}
\end{table}
